CUPID: A Real-Time Session-Based Reciprocal Recommendation System for a One-on-One Social Discovery Platform

This study introduces CUPID, a novel approach to session-based reciprocal recommendation systems designed for a real-time one-on-one social discovery platform. In such platforms, low latency is critical to enhance user experiences. However, conventional session-based approaches struggle with high latency due to the demands of modeling sequential user behavior for each recommendation process. Additionally, given the reciprocal nature of the platform, where users act as items for each other, training recommendation models on large-scale datasets is computationally prohibitive using conventional methods. To address these challenges, CUPID decouples the time-intensive user session modeling from the real-time user matching process to reduce inference time. Furthermore, CUPID employs a two-phase training strategy that separates the training of embedding and prediction layers, significantly reducing the computational burden by decreasing the number of sequential model inferences by several hundredfold. Extensive experiments on large-scale Azar datasets demonstrate CUPID's effectiveness in a real-world production environment. Notably, CUPID reduces response latency by more than 76% compared to non-asynchronous systems, while significantly improving user engagement.

==> Figures/6_latency.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{.495\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics[width=\textwidth]{Figures/6_1_latency_fig.pdf}
  }
  \vspace{-2em}
  \label{fig:6_1_latency_99}
  \caption{99th Percentiles}
\end{subfigure}%
\begin{subfigure}{.495\textwidth}
  \centering
  \resizebox{\textwidth}{!}{\includegraphics[width=\textwidth]{Figures/6_2_latency_fig.pdf}}
  \vspace{-2em}
  \label{fig:6_2_latency_90}
  \caption{90th Percentiles}
\end{subfigure}%
\caption{Response latency of \textsc{Cupid} in real-world deployment environments. Our \textsc{Cupid} can save more than 76\% of response latency compared to computing session representations synchronously in the matching pipeline.}
\label{fig:6_latency}
\end{figure*}

==> sections/6_discussion.tex <==
\section{Discussion}\label{sec:6_discussion}
In this study, we introduce our recommendation system and design experiments by employing chat duration among users as a proxy for user satisfaction scores. 
Additionally, our recommendation system is designed to predict chat duration using user features, including user demographic information (\textit{e.g.}, age and gender).
However, recent studies~\cite{singh2018fairness,biega2018equity,geyik2019fairness} argue that machine learning-based recommendation systems may provide unfair recommendation results to specific individuals or user groups when utilizing their demographic information to provide recommendations. 
Therefore, it is desirable to delicately design user satisfaction of real-time social discovery to provide fair recommendation results to individual users or user groups.
This is especially critical in reciprocal recommendations where users become targets of other users' recommendations.
Furthermore, in addition to maximizing the sum of user satisfaction scores in a matching pool, the recommendation system should connect users in a way that fairly distributes user satisfaction across users, considering the fairness of the recommendation system. 
In future research, we plan to address an improved definition of user satisfaction that can further enhance the user experience by considering ethical considerations. 
We will also design a fair matching system that can distribute user satisfaction fairly across users.
